Investigating Content Planning for Navigating Trade-offs in Knowledge-Grounded Dialogue

Knowledge-grounded dialogue generation is a challenging task because it requires satisfying two fundamental yet often competing constraints: being responsive in a manner that is specific to what the conversation partner has said while also being attributable to an underlying source document. In this work, we bring this trade-off between these two objectives (specificity and attribution) to light and ask the question: Can explicit content planning before the response generation help the model to address this challenge? To answer this question, we design a framework called PLEDGE, which allows us to experiment with various plan variables explored in prior work, supporting both metric-agnostic and metric-aware approaches. While content planning shows promise, our results on whether it can actually help to navigate this trade-off are mixed -- planning mechanisms that are metric-aware (use automatic metrics during training) are better at automatic evaluations but underperform in human judgment compared to metric-agnostic mechanisms. We discuss how this may be caused by over-fitting to automatic metrics and the need for future work to better calibrate these metrics towards human judgment. We hope the observations from our analysis will inform future work that aims to apply content planning in this context.

==> example_out_beam/ctrl.tex <==
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue."], "fact": "the royal blue was the baltimore and ohio railroad (b&o)'s flagship passenger train between new york city and washington, d.c., in the united states, beginning in 1890.", "response": "the royal blue was the baltimore and ohio railroad's flagship passenger train.", "reference": "i once road on the royal blue train from new york to d.c", "factuality_nli": 3.750562906265259}
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue.", "i once road on the royal blue train from new york to d.c", "oh that sounds really nice. i bet there was a lot of scenery and blue skies."], "fact": "blue skies is a 1946 american musical comedy film directed by stuart heisler and starring bing crosby, fred astaire, and joan caulfield.", "response": "blue skies is a 1946 american musical comedy film directed by stuart heisler and starring bing crosby, fred astaire, and joan caulfield.", "reference": "yes, speaking of blue skies, have you seen the 1946 movie staring bing crosby?", "factuality_nli": 3.900954484939575}
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue.", "i once road on the royal blue train from new york to d.c", "oh that sounds really nice. i bet there was a lot of scenery and blue skies.", "yes, speaking of blue skies, have you seen the 1946 movie staring bing crosby?", "no i haven't, but i always like the way he danced."], "fact": "harry lillis \"bing\" crosby jr. (; may 3, 1903\u00a0\u2013 october 14, 1977) was an american singer and actor.", "response": "he was an american singer and actor.", "reference": "yes. i was sad when he died in 1977. he was my favorite actor.", "factuality_nli": 3.4682960510253906}
{"context": ["hi buddy, what you think about cinematography"], "fact": "cinematography (also called \"direction of photography\") is the science or art of motion-picture photography by recording light or other electromagnetic radiation, either electronically by means of an image sensor, or chemically by means of a light-sensitive material such as film stock.", "response": "it is the science or art of motion-picture photography by recording light or other electromagnetic radiation", "reference": "cinematography,is a type of motion picture , captured electronically by means of an image", "factuality_nli": 3.64510440826416}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion."], "fact": "typically, a lens is used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface inside a camera during a questioned exposure, creating multiple images.", "response": "typically, a lens is used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface inside a camera", "reference": "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "factuality_nli": 3.9343953132629395}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", " muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks"], "fact": "photography is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor, or chemically by means of a light-sensitive material such as photographic film.", "response": "photography is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation", "reference": "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "factuality_nli": 4.030572891235352}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks", "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "yes , cinematography finds uses in many fields of science and business as well as for entertainment purposes"], "fact": "a digital camera or digicam is a camera that captures photographs in digital memory.", "response": "a digital camera or digicam is a camera that captures photographs in digital memory.", "reference": "some however prefer using   digital camera or digicam ,which is a camera that captures photograph.", "factuality_nli": 3.9455533027648926}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks", "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "yes , cinematography finds uses in many fields of science and business as well as for entertainment purposes", "some however prefer using   digital camera or digicam ,which is a camera that captures photograph.", "yes now digital camera is trendy"], "fact": "until the advent of such technology, photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical solutions to develop and stabilize the image.", "response": "until the advent of such technology, photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical solutions to develop and stabilize the image.", "reference": "prior to the advent of digital technology,  photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical .", "factuality_nli": 3.6069302558898926}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?"], "fact": "a genius is a person who displays exceptional intellectual ability, creative productivity, universality in genres or originality, typically to a degree that is associated with the achievement of new advances in a domain of knowledge.", "response": "a genius's creative productivity, universality in genres or originality, typically to a degree that is associated with the achievement of new advances in a domain of knowledge.", "reference": "universality in genres or originality typically to a degree that is associated with  achievements", "factuality_nli": 4.076446533203125}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?"], "fact": "there is no scientifically precise definition of genius, and the question of whether the notion itself has any real meaning has long been a subject of debate, although psychologists are converging on a definition that emphasizes creativity and eminent achievement.", "response": "there is no scientifically precise definition of genius, and the question of whether the notion itself has any real meaning has long been a subject of debate", "reference": "there is no scientifically precise definition of genius", "factuality_nli": 4.255074501037598}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?", "there is no scientifically precise definition of genius", "are there organizations or anything that you could belong to if you were a genius?"], "fact": "because the achievements of exceptional individuals seemed to indicate the presence of a particularly powerful \"genius\", by the time of augustus, the word began to acquire its secondary meaning of \"inspiration, talent\".", "response": "by the time of augustus, the word began to acquire its secondary meaning of \"inspiration, talent\".", "reference": "the world began to acquire its secondary meaning of inspiration, talent", "factuality_nli": 3.6438181400299072}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?", "there is no scientifically precise definition of genius", "are there organizations or anything that you could belong to if you were a genius?", "the world began to acquire its secondary meaning of inspiration, talent", "was albert enstein a genius?"], "fact": "the noun is related to the latin verb \"genui, genitus\", \"to bring into being, create, produce\", as well as to the greek word for birth.", "response": "the noun is related to the latin verb \"genui, genitus\", \"to bring into being, create, produce\"", "reference": "genius word is greed word for birth", "factuality_nli": 3.7850570678710938}
{"context": ["i just got a husky puppy"], "fact": "husky is a general name for a sled-type of dog used in northern regions, differentiated from other sled-dog types by their fast pulling style.", "response": "husky is a general name for a sled-type of dog used in northern regions", "reference": "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "factuality_nli": 3.925452947616577}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?"], "fact": "sled dogs were important for transportation in arctic areas, hauling supplies in areas that were inaccessible by other methods.", "response": "yes, they were important for transportation in the arctic regions.", "reference": "sled dogs, including huskies, are used for transportation in arctic areas.", "factuality_nli": 2.816169261932373}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?", "sled dogs, including huskies, are used for transportation in arctic areas.", "that is so cool and probably helpful but mine is just a pet "], "fact": "huskies are also today kept as pets, and groups work to find new pet homes for retired racing and adventure trekking dogs.", "response": "huskies are also kept as pets, and groups work to find new pet homes for retired racing and adventure trekking dogs.", "reference": "that's not uncommon! there are rescue groups that specialize in finding homes for retired sled dogs.", "factuality_nli": 4.213179588317871}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?", "sled dogs, including huskies, are used for transportation in arctic areas.", "that is so cool and probably helpful but mine is just a pet", "that's not uncommon! there are rescue groups that specialize in finding homes for retired sled dogs.", "i bet they retire them at a certain age then they need a home huh"], "fact": "the word \"husky\" originated from the word referring to arctic people in general, eskimos (a.k.a.", "response": "the word \"husky\" refers to arctic people in general.", "reference": "yes. huskies got their name from the word referring to eskimos.", "factuality_nli": 1.642787218093872}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things"], "fact": "it is a spontaneous or gradual process in which old memories are unable to be recalled from memory storage.", "response": "it is a spontaneous or gradual process", "reference": "its a gradual process where one is unable to call up the older memories", "factuality_nli": 3.3428280353546143}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things", "its a gradual process where one is unable to call up the older memories", "yep they just fade away and it can really get to you after a while"], "fact": "problems with remembering, learning and retaining new information are a few of the most common complaints of older adults.", "response": "remembering, learning and retaining new information are a few of the most common complaints", "reference": "memory problems are one of the most common complaints of older adults", "factuality_nli": 3.6011459827423096}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things", "its a gradual process where one is unable to call up the older memories", "yep they just fade away and it can really get to you after a while", "memory problems are one of the most common complaints of older adults", "alzheimer's is one of the worst diseases of all time."], "fact": "many different factors influence the actual process of forgetting.", "response": "yea and many different factors influence the actual process of forgetting", "reference": "alzheimers is terrible but there are many different factors that can affect the process of \"forgetting\"", "factuality_nli": 2.647773265838623}
{"context": ["i think budweiser taste terrible. have you ever had it?"], "fact": "produced in various breweries around the world, budweiser is a filtered beer available in draft and packaged forms.", "response": "it is produced in various breweries around the world, budweiser is a filtered beer available in draft", "reference": "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "factuality_nli": 3.905010461807251}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company. "], "fact": "in the european union, excluding the united kingdom, republic of ireland, sweden, finland and spain, the american beer is marketed as \"bud\", as the budweiser trademark name is owned solely by the czech beer maker, budweiser budvar.", "response": "in the european union, excluding the united kingdom, republic of ireland, sweden, finland and spain, the american beer is marketed as \"bud\", as the budweiser trademark name is owned solely by the czech beer maker", "reference": "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "factuality_nli": 3.9610276222229004}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down."], "fact": "budweiser () is an american-style pale lager produced by anheuser-busch, currently part of the transnational corporation anheuser-busch inbev.", "response": "budweiser is an american-style pale lager produced by anheuser-busch", "reference": "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "factuality_nli": 3.9303231239318848}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down.", "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "ah my favorite kind of beer are the stouts. like a nice milk or chocolate stout with a much larger alcohol content. "], "fact": "it is made with up to 30% rice in addition to hops and barley malt.", "response": "yes, and it's made with up to 30% rice in addition to hops and barley malt", "reference": "that sounds yummy!  interestingly, budweiser is made with hops and barley malt, with  up to 30% rice as well", "factuality_nli": 3.2965128421783447}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down.", "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "ah my favorite kind of beer are the stouts. like a nice milk or chocolate stout with a much larger alcohol content.", "that sounds yummy!  interestingly, budweiser is made with hops and barley malt, with  up to 30% rice as well", "oh i didn't know they used rice in their beer. i figured that was all barley, wheat and hops."], "fact": "in 1876, adolphus busch and his friend carl conrad, a liquor importer, developed a \"bohemian-style\" lager in the united states, inspired after a trip to the region.", "response": "adolphus busch and his friend carl conrad, a liquor importer, developed a \"bohemian-style\" lager in the united states", "reference": "yes, and it is a bohemian-style lager developed by adolphus busch and his friend carl conrad", "factuality_nli": 3.900242328643799}
{"context": ["who founded coors brewing company?"], "fact": "in 1873, german immigrants adolph coors and jacob schueler from prussia emigrated to the united states and established a brewery in golden, colorado, after buying a recipe for a pilsner-style beer from a czech immigrant william silhan.", "response": "1873, german immigrants adolph coors and jacob schueler from prussia emigrated to the united states", "reference": "in 1873 adolph coors and jacob schueler founded the brewery", "factuality_nli": 3.818507194519043}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?"], "fact": "it was first produced in 1978 by the coors brewing company.", "response": "it was first produced in 1978", "reference": "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "factuality_nli": 3.7646842002868652}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?", "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "what share of the market for beer did they capture ?"], "fact": "the coors brewing company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "response": "they are a regional division of the world's third-largest brewing company, the molson coors brewing company.", "reference": "i don't know the exact amount but i do know that the company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "factuality_nli": 3.8728859424591064}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?", "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "what share of the market for beer did they capture ?", "i don't know the exact amount but i do know that the company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "wow, that a huge one, thanks for enlightening me about coors brewing company"], "fact": "it is the world's seventh largest brewer by volume.", "response": "it is the world's seventh largest brewer by volume.", "reference": "oh no problem, the molson coors brewing co that was formed in 2005 is now the coors brewing company.", "factuality_nli": 3.9247193336486816}
{"context": ["i love italian cuisine"], "fact": "it has developed through centuries of social and economic changes, with roots stretching to antiquity.", "response": "it has developed through centuries of social and economic changes.", "reference": "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "factuality_nli": 4.139150619506836}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?"], "fact": "other variations found outside italy may include chicken, veal, or another type of meat cutlet or vegetable filling.", "response": "there are a lot of variations, like chicken or veal.", "reference": "i really enjoy chicken parmigiana.  what about you?", "factuality_nli": 3.004091262817383}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?", "i really enjoy chicken parmigiana.  what about you?", "i love chicken parmigiana as well, but i think my ultimate favorite is beef lasagna...extra cheese please!"], "fact": "it consists of a breaded chicken breast topped with tomato sauce and mozzarella, parmesan or provolone cheese.", "response": "it consists of breaded chicken breast topped with tomato sauce and mozzarella, parmesan or provolone cheese.", "reference": "chicken with sauce and mozzarella.... be still my heart!", "factuality_nli": 3.956796646118164}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?", "i really enjoy chicken parmigiana.  what about you?", "i love chicken parmigiana as well, but i think my ultimate favorite is beef lasagna...extra cheese please!", "chicken with sauce and mozzarella.... be still my heart!", "truthfully, anything with cheese is the best"], "fact": "it is the second-most popular cheese in the us (behind mozzarella), with an average annual consumption of per capita.", "response": "mozzarella is the second most popular cheese in the us.", "reference": "especially cheddar cheese!  it's the second most popular cheese in the us!", "factuality_nli": -0.08574120700359344}
{"context": ["my favorite color is purple, do you know much about that color?"], "fact": "purple is a color intermediate between blue and red.", "response": "purple is a color between blue and red", "reference": "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "factuality_nli": 3.4015069007873535}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?"], "fact": "according to surveys in europe and the u.s., purple is the color most often associated with royalty, magic, mystery and piety.", "response": "it is often associated with royalty, magic, mystery and piety.", "reference": "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "factuality_nli": 3.136084794998169}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?", "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "wow that's really neat. do you know what wavelengths of light purple occurs at?"], "fact": "it is similar to violet, but unlike violet, which is a spectral color with its own wavelength on the visible spectrum of light, purple is a composite color made by combining red and blue.", "response": "it is actually a composite color made by combining red and blue.", "reference": "i'm not sure exactly what wavelengths it occurs at. i do know that purple is similar to violet but unlike that spectral color it is a composite color.", "factuality_nli": 2.8494420051574707}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?", "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "wow that's really neat. do you know what wavelengths of light purple occurs at?", "i'm not sure exactly what wavelengths it occurs at. i do know that purple is similar to violet but unlike that spectral color it is a composite color.", "what exactly is a composite color, can you explain that a bit more?"], "fact": "purple is a color intermediate between blue and red.", "response": "it is a color intermediate between blue and red.", "reference": "composite means that purple is a simple color made by combining red and blue. violet is different because it's spectral.", "factuality_nli": 3.2937192916870117}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd."], "fact": "while the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j.\u00a0r.\u00a0r.\u00a0tolkien, in particular \"the lord of the rings\".", "response": "while the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j. r. r. tolkien", "reference": "while the concept remains the same it draws on many preexisting mythology", "factuality_nli": 2.146923303604126}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd.", "while the concept remains the same it draws on many preexisting mythology", "that's really interesting! orcs are some of my favorite fictional characters honestly."], "fact": "while the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j.\u00a0r.\u00a0r.\u00a0tolkien, in particular \"the lord of the rings\".", "response": "the main conception of the creatures stems from the fantasy writings of j. r. r. tolkien", "reference": "orcs were actually created by j r r tolkein", "factuality_nli": 2.4736995697021484}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd.", "while the concept remains the same it draws on many preexisting mythology", "that's really interesting! orcs are some of my favorite fictional characters honestly.", "orcs were actually created by j r r tolkein", "really? cool, i'll have to look him up sometime."], "fact": "an orc (also spelled as ork) is a fictional humanoid creature that is part of a fantasy race akin to goblins.", "response": "ork) is a fictional humanoid creature that is part of a fantasy race akin to goblins", "reference": "orcs are very similar to thinks like goblins and are a humanoid race", "factuality_nli": 2.2556018829345703}


==> example_out_beam/noctrl.tex <==
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue."], "fact": "the royal blue was the baltimore and ohio railroad (b&o)'s flagship passenger train between new york city and washington, d.c., in the united states, beginning in 1890.", "response": "the royal blue was the baltimore and ohio railroad's flagship passenger train.", "reference": "i once road on the royal blue train from new york to d.c", "factuality_nli": 3.750562906265259}
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue.", "i once road on the royal blue train from new york to d.c", "oh that sounds really nice. i bet there was a lot of scenery and blue skies."], "fact": "blue skies is a 1946 american musical comedy film directed by stuart heisler and starring bing crosby, fred astaire, and joan caulfield.", "response": "blue skies is a 1946 american musical comedy film", "reference": "yes, speaking of blue skies, have you seen the 1946 movie staring bing crosby?", "factuality_nli": 3.6190502643585205}
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue.", "i once road on the royal blue train from new york to d.c", "oh that sounds really nice. i bet there was a lot of scenery and blue skies.", "yes, speaking of blue skies, have you seen the 1946 movie staring bing crosby?", "no i haven't, but i always like the way he danced."], "fact": "harry lillis \"bing\" crosby jr. (; may 3, 1903\u00a0\u2013 october 14, 1977) was an american singer and actor.", "response": "bing crosby jr. was an american singer and actor.", "reference": "yes. i was sad when he died in 1977. he was my favorite actor.", "factuality_nli": 3.7747745513916016}
{"context": ["hi buddy, what you think about cinematography"], "fact": "cinematography (also called \"direction of photography\") is the science or art of motion-picture photography by recording light or other electromagnetic radiation, either electronically by means of an image sensor, or chemically by means of a light-sensitive material such as film stock.", "response": "cinematography is the science or art of motion-picture photography", "reference": "cinematography,is a type of motion picture , captured electronically by means of an image", "factuality_nli": 3.0083601474761963}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion."], "fact": "typically, a lens is used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface inside a camera during a questioned exposure, creating multiple images.", "response": "typically, a lens is used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface inside a camera", "reference": "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "factuality_nli": 3.9343953132629395}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", " muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks"], "fact": "photography is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor, or chemically by means of a light-sensitive material such as photographic film.", "response": "photography is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation", "reference": "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "factuality_nli": 4.030572891235352}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks", "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "yes , cinematography finds uses in many fields of science and business as well as for entertainment purposes"], "fact": "a digital camera or digicam is a camera that captures photographs in digital memory.", "response": "a digital camera or digicam is a camera that captures photographs in digital memory.", "reference": "some however prefer using   digital camera or digicam ,which is a camera that captures photograph.", "factuality_nli": 3.9455533027648926}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks", "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "yes , cinematography finds uses in many fields of science and business as well as for entertainment purposes", "some however prefer using   digital camera or digicam ,which is a camera that captures photograph.", "yes now digital camera is trendy"], "fact": "until the advent of such technology, photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical solutions to develop and stabilize the image.", "response": "before the advent of such technology, photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical solutions to develop and stabilize the image.", "reference": "prior to the advent of digital technology,  photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical .", "factuality_nli": 3.875462055206299}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?"], "fact": "a genius is a person who displays exceptional intellectual ability, creative productivity, universality in genres or originality, typically to a degree that is associated with the achievement of new advances in a domain of knowledge.", "response": "exceptional intellectual ability, creative productivity, universality in genres or originality, typically to a degree that is associated with the achievement of new advances in a domain of knowledge.", "reference": "universality in genres or originality typically to a degree that is associated with  achievements", "factuality_nli": 3.9455864429473877}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?"], "fact": "there is no scientifically precise definition of genius, and the question of whether the notion itself has any real meaning has long been a subject of debate, although psychologists are converging on a definition that emphasizes creativity and eminent achievement.", "response": "there is no scientifically precise definition of genius, and the question of whether the notion itself has any real meaning", "reference": "there is no scientifically precise definition of genius", "factuality_nli": 3.999898910522461}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?", "there is no scientifically precise definition of genius", "are there organizations or anything that you could belong to if you were a genius?"], "fact": "because the achievements of exceptional individuals seemed to indicate the presence of a particularly powerful \"genius\", by the time of augustus, the word began to acquire its secondary meaning of \"inspiration, talent\".", "response": "by the time of augustus, the word began to acquire its secondary meaning \"inspiration, talent\".", "reference": "the world began to acquire its secondary meaning of inspiration, talent", "factuality_nli": 3.6375246047973633}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?", "there is no scientifically precise definition of genius", "are there organizations or anything that you could belong to if you were a genius?", "the world began to acquire its secondary meaning of inspiration, talent", "was albert enstein a genius?"], "fact": "the noun is related to the latin verb \"genui, genitus\", \"to bring into being, create, produce\", as well as to the greek word for birth.", "response": "yes he was. the noun is related to the latin verb \"genui, genitus\", \"to bring into being, create, produce\"", "reference": "genius word is greed word for birth", "factuality_nli": -0.022556737065315247}
{"context": ["i just got a husky puppy"], "fact": "husky is a general name for a sled-type of dog used in northern regions, differentiated from other sled-dog types by their fast pulling style.", "response": "husky is a general name for a sled-type of dog used in northern regions", "reference": "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "factuality_nli": 3.925452947616577}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?"], "fact": "sled dogs were important for transportation in arctic areas, hauling supplies in areas that were inaccessible by other methods.", "response": "yes, sled dogs were important for transportation in the arctic.", "reference": "sled dogs, including huskies, are used for transportation in arctic areas.", "factuality_nli": 3.3297948837280273}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?", "sled dogs, including huskies, are used for transportation in arctic areas.", "that is so cool and probably helpful but mine is just a pet "], "fact": "huskies are also today kept as pets, and groups work to find new pet homes for retired racing and adventure trekking dogs.", "response": "huskies are also kept as pets, and groups work to find new pet homes for retired racing and adventure trekking dogs.", "reference": "that's not uncommon! there are rescue groups that specialize in finding homes for retired sled dogs.", "factuality_nli": 4.213179588317871}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?", "sled dogs, including huskies, are used for transportation in arctic areas.", "that is so cool and probably helpful but mine is just a pet", "that's not uncommon! there are rescue groups that specialize in finding homes for retired sled dogs.", "i bet they retire them at a certain age then they need a home huh"], "fact": "the word \"husky\" originated from the word referring to arctic people in general, eskimos (a.k.a.", "response": "yes! the word \"husky\" originated from the word referring to arctic people.", "reference": "yes. huskies got their name from the word referring to eskimos.", "factuality_nli": 2.2250208854675293}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things"], "fact": "it is a spontaneous or gradual process in which old memories are unable to be recalled from memory storage.", "response": "it is a spontaneous or gradual process in which old memories are unable to be recalled from memory storage.", "reference": "its a gradual process where one is unable to call up the older memories", "factuality_nli": 4.014892101287842}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things", "its a gradual process where one is unable to call up the older memories", "yep they just fade away and it can really get to you after a while"], "fact": "problems with remembering, learning and retaining new information are a few of the most common complaints of older adults.", "response": "memory loss is one of the most common complaints of older adults", "reference": "memory problems are one of the most common complaints of older adults", "factuality_nli": 4.008386611938477}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things", "its a gradual process where one is unable to call up the older memories", "yep they just fade away and it can really get to you after a while", "memory problems are one of the most common complaints of older adults", "alzheimer's is one of the worst diseases of all time."], "fact": "many different factors influence the actual process of forgetting.", "response": "many different factors influence the actual process of forgetting", "reference": "alzheimers is terrible but there are many different factors that can affect the process of \"forgetting\"", "factuality_nli": 4.195316314697266}
{"context": ["i think budweiser taste terrible. have you ever had it?"], "fact": "produced in various breweries around the world, budweiser is a filtered beer available in draft and packaged forms.", "response": "budweiser is a filtered beer produced in various breweries around the world", "reference": "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "factuality_nli": 3.9650583267211914}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company. "], "fact": "in the european union, excluding the united kingdom, republic of ireland, sweden, finland and spain, the american beer is marketed as \"bud\", as the budweiser trademark name is owned solely by the czech beer maker, budweiser budvar.", "response": "in the european union, excluding the united kingdom, republic of ireland, sweden, finland and spain, the american beer is marketed as \"bud\"", "reference": "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "factuality_nli": 3.8745551109313965}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down."], "fact": "budweiser () is an american-style pale lager produced by anheuser-busch, currently part of the transnational corporation anheuser-busch inbev.", "response": "budweiser is an american-style pale lager produced by anheuser-busch", "reference": "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "factuality_nli": 3.9303231239318848}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down.", "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "ah my favorite kind of beer are the stouts. like a nice milk or chocolate stout with a much larger alcohol content. "], "fact": "it is made with up to 30% rice in addition to hops and barley malt.", "response": "i love stouts too! they are made with up to 30% rice in addition to hops and barley malt", "reference": "that sounds yummy!  interestingly, budweiser is made with hops and barley malt, with  up to 30% rice as well", "factuality_nli": -1.9625685214996338}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down.", "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "ah my favorite kind of beer are the stouts. like a nice milk or chocolate stout with a much larger alcohol content.", "that sounds yummy!  interestingly, budweiser is made with hops and barley malt, with  up to 30% rice as well", "oh i didn't know they used rice in their beer. i figured that was all barley, wheat and hops."], "fact": "in 1876, adolphus busch and his friend carl conrad, a liquor importer, developed a \"bohemian-style\" lager in the united states, inspired after a trip to the region.", "response": "interestingly, in 1876, adolphus busch and his friend carl conrad, a liquor importer, developed a \"bohemian-style\" lager in the united states, inspired by a trip to the region", "reference": "yes, and it is a bohemian-style lager developed by adolphus busch and his friend carl conrad", "factuality_nli": 2.7206273078918457}
{"context": ["who founded coors brewing company?"], "fact": "in 1873, german immigrants adolph coors and jacob schueler from prussia emigrated to the united states and established a brewery in golden, colorado, after buying a recipe for a pilsner-style beer from a czech immigrant william silhan.", "response": "in 1873, german immigrants adolph coors and jacob schueler from prussia emigrated to the united states and established a brewery in golden, colorado.", "reference": "in 1873 adolph coors and jacob schueler founded the brewery", "factuality_nli": 4.083568572998047}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?"], "fact": "it was first produced in 1978 by the coors brewing company.", "response": "beer. it was first produced in 1978 by the coors brewing company.", "reference": "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "factuality_nli": 1.089069128036499}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?", "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "what share of the market for beer did they capture ?"], "fact": "the coors brewing company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "response": "the coors brewing company is a regional division of the world's third largest brewing company.", "reference": "i don't know the exact amount but i do know that the company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "factuality_nli": 3.7629165649414062}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?", "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "what share of the market for beer did they capture ?", "i don't know the exact amount but i do know that the company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "wow, that a huge one, thanks for enlightening me about coors brewing company"], "fact": "it is the world's seventh largest brewer by volume.", "response": "it is the world's seventh largest brewer by volume.", "reference": "oh no problem, the molson coors brewing co that was formed in 2005 is now the coors brewing company.", "factuality_nli": 3.9247193336486816}
{"context": ["i love italian cuisine"], "fact": "it has developed through centuries of social and economic changes, with roots stretching to antiquity.", "response": "i love it too, it has developed through centuries of social and economic changes", "reference": "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "factuality_nli": -1.1995487213134766}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?"], "fact": "other variations found outside italy may include chicken, veal, or another type of meat cutlet or vegetable filling.", "response": "i love anything with meat or vegetables.", "reference": "i really enjoy chicken parmigiana.  what about you?", "factuality_nli": -1.9472707509994507}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?", "i really enjoy chicken parmigiana.  what about you?", "i love chicken parmigiana as well, but i think my ultimate favorite is beef lasagna...extra cheese please!"], "fact": "it consists of a breaded chicken breast topped with tomato sauce and mozzarella, parmesan or provolone cheese.", "response": "oh yes, i love beef lasagna. it's breaded chicken breast topped with mozzarella, parmesan or provolone cheese.", "reference": "chicken with sauce and mozzarella.... be still my heart!", "factuality_nli": -0.5287802815437317}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?", "i really enjoy chicken parmigiana.  what about you?", "i love chicken parmigiana as well, but i think my ultimate favorite is beef lasagna...extra cheese please!", "chicken with sauce and mozzarella.... be still my heart!", "truthfully, anything with cheese is the best"], "fact": "it is the second-most popular cheese in the us (behind mozzarella), with an average annual consumption of per capita.", "response": "cheese is the second most popular cheese in the us!", "reference": "especially cheddar cheese!  it's the second most popular cheese in the us!", "factuality_nli": 2.9982833862304688}
{"context": ["my favorite color is purple, do you know much about that color?"], "fact": "purple is a color intermediate between blue and red.", "response": "purple is a color intermediate between blue and red.", "reference": "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "factuality_nli": 3.8220951557159424}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?"], "fact": "according to surveys in europe and the u.s., purple is the color most often associated with royalty, magic, mystery and piety.", "response": "according to surveys in europe and the u.s., purple is the color most often associated with royalty, magic, mystery and piety.", "reference": "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "factuality_nli": 4.016571044921875}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?", "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "wow that's really neat. do you know what wavelengths of light purple occurs at?"], "fact": "it is similar to violet, but unlike violet, which is a spectral color with its own wavelength on the visible spectrum of light, purple is a composite color made by combining red and blue.", "response": "i do not, but i do know that it is similar to violet, but unlike violet, which is a spectral color with its own wavelength on the visible spectrum of light, purple is a composite color made by combining red and blue.", "reference": "i'm not sure exactly what wavelengths it occurs at. i do know that purple is similar to violet but unlike that spectral color it is a composite color.", "factuality_nli": -1.0221784114837646}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?", "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "wow that's really neat. do you know what wavelengths of light purple occurs at?", "i'm not sure exactly what wavelengths it occurs at. i do know that purple is similar to violet but unlike that spectral color it is a composite color.", "what exactly is a composite color, can you explain that a bit more?"], "fact": "purple is a color intermediate between blue and red.", "response": "it is a color intermediate between blue and red.", "reference": "composite means that purple is a simple color made by combining red and blue. violet is different because it's spectral.", "factuality_nli": 3.2937192916870117}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd."], "fact": "while the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j.\u00a0r.\u00a0r.\u00a0tolkien, in particular \"the lord of the rings\".", "response": "while the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j. r. r. tolkien", "reference": "while the concept remains the same it draws on many preexisting mythology", "factuality_nli": 2.146923303604126}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd.", "while the concept remains the same it draws on many preexisting mythology", "that's really interesting! orcs are some of my favorite fictional characters honestly."], "fact": "while the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j.\u00a0r.\u00a0r.\u00a0tolkien, in particular \"the lord of the rings\".", "response": "the main conception of the creatures stems from the fantasy writings of j. r. r. tolkien", "reference": "orcs were actually created by j r r tolkein", "factuality_nli": 2.4736995697021484}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd.", "while the concept remains the same it draws on many preexisting mythology", "that's really interesting! orcs are some of my favorite fictional characters honestly.", "orcs were actually created by j r r tolkein", "really? cool, i'll have to look him up sometime."], "fact": "an orc (also spelled as ork) is a fictional humanoid creature that is part of a fantasy race akin to goblins.", "response": "an orc is a fictional humanoid creature that is part of a fantasy race akin to goblins", "reference": "orcs are very similar to thinks like goblins and are a humanoid race", "factuality_nli": 3.8956902027130127}

==> example_out_beam/plan-full-0e.tex <==
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue."], "fact": "the royal blue was the baltimore and ohio railroad (b&o)'s flagship passenger train between new york city and washington, d.c., in the united states, beginning in 1890.", "response": "the royal blue was the baltimore and ohio railroad's flagship passenger train between new york city and washington", "reference": "i once road on the royal blue train from new york to d.c", "factuality_nli": 3.7813332080841064}
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue.", "i once road on the royal blue train from new york to d.c", "oh that sounds really nice. i bet there was a lot of scenery and blue skies."], "fact": "blue skies is a 1946 american musical comedy film directed by stuart heisler and starring bing crosby, fred astaire, and joan caulfield.", "response": "blue skies was a 1946 american musical comedy film directed by stuart heisler and starring bing crosby", "reference": "yes, speaking of blue skies, have you seen the 1946 movie staring bing crosby?", "factuality_nli": 3.607492446899414}
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue.", "i once road on the royal blue train from new york to d.c", "oh that sounds really nice. i bet there was a lot of scenery and blue skies.", "yes, speaking of blue skies, have you seen the 1946 movie staring bing crosby?", "no i haven't, but i always like the way he danced."], "fact": "harry lillis \"bing\" crosby jr. (; may 3, 1903\u00a0\u2013 october 14, 1977) was an american singer and actor.", "response": "he was harry lillis \"bing\" crosby jr.", "reference": "yes. i was sad when he died in 1977. he was my favorite actor.", "factuality_nli": 2.2567801475524902}
{"context": ["hi buddy, what you think about cinematography"], "fact": "cinematography (also called \"direction of photography\") is the science or art of motion-picture photography by recording light or other electromagnetic radiation, either electronically by means of an image sensor, or chemically by means of a light-sensitive material such as film stock.", "response": "cinematography is the science or art of motion-picture photography", "reference": "cinematography,is a type of motion picture , captured electronically by means of an image", "factuality_nli": 3.0083601474761963}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion."], "fact": "typically, a lens is used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface inside a camera during a questioned exposure, creating multiple images.", "response": "typically, a lens is used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface inside a camera", "reference": "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "factuality_nli": 3.9343953132629395}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", " muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks"], "fact": "photography is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor, or chemically by means of a light-sensitive material such as photographic film.", "response": "photography is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation", "reference": "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "factuality_nli": 4.030572891235352}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks", "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "yes , cinematography finds uses in many fields of science and business as well as for entertainment purposes"], "fact": "a digital camera or digicam is a camera that captures photographs in digital memory.", "response": "a digital camera or digicam is a camera that captures photographs in digital memory.", "reference": "some however prefer using   digital camera or digicam ,which is a camera that captures photograph.", "factuality_nli": 3.9455533027648926}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks", "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "yes , cinematography finds uses in many fields of science and business as well as for entertainment purposes", "some however prefer using   digital camera or digicam ,which is a camera that captures photograph.", "yes now digital camera is trendy"], "fact": "until the advent of such technology, photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical solutions to develop and stabilize the image.", "response": "until the advent of such technology, photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical solutions to develop and stabilize the image.", "reference": "prior to the advent of digital technology,  photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical .", "factuality_nli": 3.6069302558898926}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?"], "fact": "a genius is a person who displays exceptional intellectual ability, creative productivity, universality in genres or originality, typically to a degree that is associated with the achievement of new advances in a domain of knowledge.", "response": "genius is a person who has exceptional creative productivity.", "reference": "universality in genres or originality typically to a degree that is associated with  achievements", "factuality_nli": 3.378361463546753}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?"], "fact": "there is no scientifically precise definition of genius, and the question of whether the notion itself has any real meaning has long been a subject of debate, although psychologists are converging on a definition that emphasizes creativity and eminent achievement.", "response": "there is no scientifically precise definition of genius", "reference": "there is no scientifically precise definition of genius", "factuality_nli": 3.760834217071533}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?", "there is no scientifically precise definition of genius", "are there organizations or anything that you could belong to if you were a genius?"], "fact": "because the achievements of exceptional individuals seemed to indicate the presence of a particularly powerful \"genius\", by the time of augustus, the word began to acquire its secondary meaning of \"inspiration, talent\".", "response": "by the time of augustus, the word began to acquire its secondary meaning \"inspiration, talent", "reference": "the world began to acquire its secondary meaning of inspiration, talent", "factuality_nli": 3.6190836429595947}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?", "there is no scientifically precise definition of genius", "are there organizations or anything that you could belong to if you were a genius?", "the world began to acquire its secondary meaning of inspiration, talent", "was albert enstein a genius?"], "fact": "the noun is related to the latin verb \"genui, genitus\", \"to bring into being, create, produce\", as well as to the greek word for birth.", "response": "the noun is related to the latin verb \"genui, genitus\", \"to bring into being, create, produce\" as well as to the greek word for birth.", "reference": "genius word is greed word for birth", "factuality_nli": 4.1075358390808105}
{"context": ["i just got a husky puppy"], "fact": "husky is a general name for a sled-type of dog used in northern regions, differentiated from other sled-dog types by their fast pulling style.", "response": "husky is a general name for a sled-type of dog used in northern regions", "reference": "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "factuality_nli": 3.925452947616577}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?"], "fact": "sled dogs were important for transportation in arctic areas, hauling supplies in areas that were inaccessible by other methods.", "response": "sled dogs were important for hauling supplies in arctic areas.", "reference": "sled dogs, including huskies, are used for transportation in arctic areas.", "factuality_nli": 4.105292797088623}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?", "sled dogs, including huskies, are used for transportation in arctic areas.", "that is so cool and probably helpful but mine is just a pet "], "fact": "huskies are also today kept as pets, and groups work to find new pet homes for retired racing and adventure trekking dogs.", "response": "huskies are also kept as pets, and groups work to find new pet homes for retired racing and adventure trekking dogs.", "reference": "that's not uncommon! there are rescue groups that specialize in finding homes for retired sled dogs.", "factuality_nli": 4.213179588317871}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?", "sled dogs, including huskies, are used for transportation in arctic areas.", "that is so cool and probably helpful but mine is just a pet", "that's not uncommon! there are rescue groups that specialize in finding homes for retired sled dogs.", "i bet they retire them at a certain age then they need a home huh"], "fact": "the word \"husky\" originated from the word referring to arctic people in general, eskimos (a.k.a.", "response": "the word \"husky\" originated from the word referring to arctic people in general, eskimos", "reference": "yes. huskies got their name from the word referring to eskimos.", "factuality_nli": 3.8653526306152344}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things"], "fact": "it is a spontaneous or gradual process in which old memories are unable to be recalled from memory storage.", "response": "it is a spontaneous or gradual process in which old memories are unable to be recalled from memory storage.", "reference": "its a gradual process where one is unable to call up the older memories", "factuality_nli": 4.014892101287842}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things", "its a gradual process where one is unable to call up the older memories", "yep they just fade away and it can really get to you after a while"], "fact": "problems with remembering, learning and retaining new information are a few of the most common complaints of older adults.", "response": "problems with remembering, learning and retaining new information are a few of the most common complaints of older adults", "reference": "memory problems are one of the most common complaints of older adults", "factuality_nli": 4.197671890258789}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things", "its a gradual process where one is unable to call up the older memories", "yep they just fade away and it can really get to you after a while", "memory problems are one of the most common complaints of older adults", "alzheimer's is one of the worst diseases of all time."], "fact": "many different factors influence the actual process of forgetting.", "response": "many different factors influence the actual process of forgetting", "reference": "alzheimers is terrible but there are many different factors that can affect the process of \"forgetting\"", "factuality_nli": 4.195316314697266}
{"context": ["i think budweiser taste terrible. have you ever had it?"], "fact": "produced in various breweries around the world, budweiser is a filtered beer available in draft and packaged forms.", "response": "i have! budweiser is produced in various breweries around the world", "reference": "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "factuality_nli": 2.186922550201416}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company. "], "fact": "in the european union, excluding the united kingdom, republic of ireland, sweden, finland and spain, the american beer is marketed as \"bud\", as the budweiser trademark name is owned solely by the czech beer maker, budweiser budvar.", "response": "budweiser budvar is owned by the czech beer maker, budweiser budvar", "reference": "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "factuality_nli": 1.9554049968719482}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down."], "fact": "budweiser () is an american-style pale lager produced by anheuser-busch, currently part of the transnational corporation anheuser-busch inbev.", "response": "budweiser is an american-style pale lager produced by anheuser-busch", "reference": "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "factuality_nli": 3.9303231239318848}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down.", "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "ah my favorite kind of beer are the stouts. like a nice milk or chocolate stout with a much larger alcohol content. "], "fact": "it is made with up to 30% rice in addition to hops and barley malt.", "response": "stouts are great! they are made with up to 30% rice in addition to hops and barley malt", "reference": "that sounds yummy!  interestingly, budweiser is made with hops and barley malt, with  up to 30% rice as well", "factuality_nli": -1.5555663108825684}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down.", "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "ah my favorite kind of beer are the stouts. like a nice milk or chocolate stout with a much larger alcohol content.", "that sounds yummy!  interestingly, budweiser is made with hops and barley malt, with  up to 30% rice as well", "oh i didn't know they used rice in their beer. i figured that was all barley, wheat and hops."], "fact": "in 1876, adolphus busch and his friend carl conrad, a liquor importer, developed a \"bohemian-style\" lager in the united states, inspired after a trip to the region.", "response": "interestingly, in 1876, adolphus busch and his friend carl conrad, a liquor importer, developed a bohemian-style lager in the united states", "reference": "yes, and it is a bohemian-style lager developed by adolphus busch and his friend carl conrad", "factuality_nli": 2.708996295928955}
{"context": ["who founded coors brewing company?"], "fact": "in 1873, german immigrants adolph coors and jacob schueler from prussia emigrated to the united states and established a brewery in golden, colorado, after buying a recipe for a pilsner-style beer from a czech immigrant william silhan.", "response": "adolph coors and jacob schueler from prussia emigrated to the united states in 1873.", "reference": "in 1873 adolph coors and jacob schueler founded the brewery", "factuality_nli": 3.917875289916992}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?"], "fact": "it was first produced in 1978 by the coors brewing company.", "response": "coors brewing company was first produced in 1978", "reference": "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "factuality_nli": 2.562623977661133}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?", "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "what share of the market for beer did they capture ?"], "fact": "the coors brewing company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "response": "the coors brewing company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "reference": "i don't know the exact amount but i do know that the company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "factuality_nli": 3.81034779548645}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?", "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "what share of the market for beer did they capture ?", "i don't know the exact amount but i do know that the company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "wow, that a huge one, thanks for enlightening me about coors brewing company"], "fact": "it is the world's seventh largest brewer by volume.", "response": "they are the world's seventh largest brewer by volume.", "reference": "oh no problem, the molson coors brewing co that was formed in 2005 is now the coors brewing company.", "factuality_nli": 3.872642993927002}
{"context": ["i love italian cuisine"], "fact": "it has developed through centuries of social and economic changes, with roots stretching to antiquity.", "response": "i love it too, it has developed through centuries of social and economic changes.", "reference": "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "factuality_nli": -1.269578218460083}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?"], "fact": "other variations found outside italy may include chicken, veal, or another type of meat cutlet or vegetable filling.", "response": "i love chicken and veal.", "reference": "i really enjoy chicken parmigiana.  what about you?", "factuality_nli": -2.0872128009796143}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?", "i really enjoy chicken parmigiana.  what about you?", "i love chicken parmigiana as well, but i think my ultimate favorite is beef lasagna...extra cheese please!"], "fact": "it consists of a breaded chicken breast topped with tomato sauce and mozzarella, parmesan or provolone cheese.", "response": "i love beef parmigiana. i love the breaded chicken breast.", "reference": "chicken with sauce and mozzarella.... be still my heart!", "factuality_nli": -1.6813510656356812}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?", "i really enjoy chicken parmigiana.  what about you?", "i love chicken parmigiana as well, but i think my ultimate favorite is beef lasagna...extra cheese please!", "chicken with sauce and mozzarella.... be still my heart!", "truthfully, anything with cheese is the best"], "fact": "it is the second-most popular cheese in the us (behind mozzarella), with an average annual consumption of per capita.", "response": "i agree. cheese is the second most popular cheese in the us.", "reference": "especially cheddar cheese!  it's the second most popular cheese in the us!", "factuality_nli": 1.8861215114593506}
{"context": ["my favorite color is purple, do you know much about that color?"], "fact": "purple is a color intermediate between blue and red.", "response": "i know that it is a color intermediate between blue and red.", "reference": "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "factuality_nli": 0.8976457118988037}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?"], "fact": "according to surveys in europe and the u.s., purple is the color most often associated with royalty, magic, mystery and piety.", "response": "it is often associated with royalty, magic, and piety.", "reference": "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "factuality_nli": 3.2820382118225098}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?", "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "wow that's really neat. do you know what wavelengths of light purple occurs at?"], "fact": "it is similar to violet, but unlike violet, which is a spectral color with its own wavelength on the visible spectrum of light, purple is a composite color made by combining red and blue.", "response": "i don't, but i do know that it is similar to violet in that it is a composite color made by combining red and blue.", "reference": "i'm not sure exactly what wavelengths it occurs at. i do know that purple is similar to violet but unlike that spectral color it is a composite color.", "factuality_nli": -0.30086803436279297}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?", "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "wow that's really neat. do you know what wavelengths of light purple occurs at?", "i'm not sure exactly what wavelengths it occurs at. i do know that purple is similar to violet but unlike that spectral color it is a composite color.", "what exactly is a composite color, can you explain that a bit more?"], "fact": "purple is a color intermediate between blue and red.", "response": "it is a color that is intermediate between blue and red.", "reference": "composite means that purple is a simple color made by combining red and blue. violet is different because it's spectral.", "factuality_nli": 3.410508871078491}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd."], "fact": "while the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j.\u00a0r.\u00a0r.\u00a0tolkien, in particular \"the lord of the rings\".", "response": "j. r. r. tolkien wrote the lord of the rings", "reference": "while the concept remains the same it draws on many preexisting mythology", "factuality_nli": 2.1027140617370605}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd.", "while the concept remains the same it draws on many preexisting mythology", "that's really interesting! orcs are some of my favorite fictional characters honestly."], "fact": "while the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j.\u00a0r.\u00a0r.\u00a0tolkien, in particular \"the lord of the rings\".", "response": "the main conception of the creatures stems from the fantasy writings of j. r. r. tolkien", "reference": "orcs were actually created by j r r tolkein", "factuality_nli": 2.4736995697021484}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd.", "while the concept remains the same it draws on many preexisting mythology", "that's really interesting! orcs are some of my favorite fictional characters honestly.", "orcs were actually created by j r r tolkein", "really? cool, i'll have to look him up sometime."], "fact": "an orc (also spelled as ork) is a fictional humanoid creature that is part of a fantasy race akin to goblins.", "response": "ork is also spelled as ork", "reference": "orcs are very similar to thinks like goblins and are a humanoid race", "factuality_nli": 2.355752468109131}

==> example_out_beam/plan-keywords-0e.tex <==
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue."], "fact": "the royal blue was the baltimore and ohio railroad (b&o)'s flagship passenger train between new york city and washington, d.c., in the united states, beginning in 1890.", "response": "the royal blue was the baltimore and ohio railroad's flagship passenger train between new york city and washington.", "reference": "i once road on the royal blue train from new york to d.c", "factuality_nli": 3.81148624420166}
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue.", "i once road on the royal blue train from new york to d.c", "oh that sounds really nice. i bet there was a lot of scenery and blue skies."], "fact": "blue skies is a 1946 american musical comedy film directed by stuart heisler and starring bing crosby, fred astaire, and joan caulfield.", "response": "blue skies was a musical comedy film directed by stuart heisler and starring bing crosby and fred astaire.", "reference": "yes, speaking of blue skies, have you seen the 1946 movie staring bing crosby?", "factuality_nli": 3.5118722915649414}
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue.", "i once road on the royal blue train from new york to d.c", "oh that sounds really nice. i bet there was a lot of scenery and blue skies.", "yes, speaking of blue skies, have you seen the 1946 movie staring bing crosby?", "no i haven't, but i always like the way he danced."], "fact": "harry lillis \"bing\" crosby jr. (; may 3, 1903\u00a0\u2013 october 14, 1977) was an american singer and actor.", "response": "bing crosby jr. was an american singer and actor.", "reference": "yes. i was sad when he died in 1977. he was my favorite actor.", "factuality_nli": 3.7747745513916016}
{"context": ["hi buddy, what you think about cinematography"], "fact": "cinematography (also called \"direction of photography\") is the science or art of motion-picture photography by recording light or other electromagnetic radiation, either electronically by means of an image sensor, or chemically by means of a light-sensitive material such as film stock.", "response": "cinematography is the science or art of motion-picture photography", "reference": "cinematography,is a type of motion picture , captured electronically by means of an image", "factuality_nli": 3.0083601474761963}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion."], "fact": "typically, a lens is used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface inside a camera during a questioned exposure, creating multiple images.", "response": "typically, a lens is used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface inside a camera", "reference": "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "factuality_nli": 3.9343953132629395}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", " muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks"], "fact": "photography is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor, or chemically by means of a light-sensitive material such as photographic film.", "response": "photography is the science, art,application and practice of creating durable images by recording light or other electromagnetic radiation", "reference": "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "factuality_nli": 3.99471378326416}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks", "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "yes , cinematography finds uses in many fields of science and business as well as for entertainment purposes"], "fact": "a digital camera or digicam is a camera that captures photographs in digital memory.", "response": "a digital camera or digicam is a camera that captures photographs in digital memory.", "reference": "some however prefer using   digital camera or digicam ,which is a camera that captures photograph.", "factuality_nli": 3.9455533027648926}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks", "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "yes , cinematography finds uses in many fields of science and business as well as for entertainment purposes", "some however prefer using   digital camera or digicam ,which is a camera that captures photograph.", "yes now digital camera is trendy"], "fact": "until the advent of such technology, photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical solutions to develop and stabilize the image.", "response": "before such technology, photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical solutions to develop and stabilize the image.", "reference": "prior to the advent of digital technology,  photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical .", "factuality_nli": 3.80971097946167}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?"], "fact": "a genius is a person who displays exceptional intellectual ability, creative productivity, universality in genres or originality, typically to a degree that is associated with the achievement of new advances in a domain of knowledge.", "response": "exceptional intellectual ability, creative productivity, universality in genres or originality.", "reference": "universality in genres or originality typically to a degree that is associated with  achievements", "factuality_nli": 3.4147729873657227}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?"], "fact": "there is no scientifically precise definition of genius, and the question of whether the notion itself has any real meaning has long been a subject of debate, although psychologists are converging on a definition that emphasizes creativity and eminent achievement.", "response": "there is no scientifically precise definition of genius", "reference": "there is no scientifically precise definition of genius", "factuality_nli": 3.760834217071533}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?", "there is no scientifically precise definition of genius", "are there organizations or anything that you could belong to if you were a genius?"], "fact": "because the achievements of exceptional individuals seemed to indicate the presence of a particularly powerful \"genius\", by the time of augustus, the word began to acquire its secondary meaning of \"inspiration, talent\".", "response": "because the achievements of exceptional individuals seemed to indicate the presence of a particularly powerful \"genius\", by the time of augustus, the word began to acquire its secondary meaning", "reference": "the world began to acquire its secondary meaning of inspiration, talent", "factuality_nli": 3.7193856239318848}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?", "there is no scientifically precise definition of genius", "are there organizations or anything that you could belong to if you were a genius?", "the world began to acquire its secondary meaning of inspiration, talent", "was albert enstein a genius?"], "fact": "the noun is related to the latin verb \"genui, genitus\", \"to bring into being, create, produce\", as well as to the greek word for birth.", "response": "the noun is related to the latin verb \"genui, genitus\", \"to bring into being, create, produce\", as well as to the greek word for birth.", "reference": "genius word is greed word for birth", "factuality_nli": 4.08937931060791}
{"context": ["i just got a husky puppy"], "fact": "husky is a general name for a sled-type of dog used in northern regions, differentiated from other sled-dog types by their fast pulling style.", "response": "husky is a general name for a sled-type of dog used in northern regions", "reference": "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "factuality_nli": 3.925452947616577}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?"], "fact": "sled dogs were important for transportation in arctic areas, hauling supplies in areas that were inaccessible by other methods.", "response": "sled dogs were important for hauling supplies in the arctic.", "reference": "sled dogs, including huskies, are used for transportation in arctic areas.", "factuality_nli": 4.1028594970703125}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?", "sled dogs, including huskies, are used for transportation in arctic areas.", "that is so cool and probably helpful but mine is just a pet "], "fact": "huskies are also today kept as pets, and groups work to find new pet homes for retired racing and adventure trekking dogs.", "response": "huskies are also kept as pets, and groups work to find new pet homes for retired racing and adventure trekking dogs.", "reference": "that's not uncommon! there are rescue groups that specialize in finding homes for retired sled dogs.", "factuality_nli": 4.213179588317871}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?", "sled dogs, including huskies, are used for transportation in arctic areas.", "that is so cool and probably helpful but mine is just a pet", "that's not uncommon! there are rescue groups that specialize in finding homes for retired sled dogs.", "i bet they retire them at a certain age then they need a home huh"], "fact": "the word \"husky\" originated from the word referring to arctic people in general, eskimos (a.k.a.", "response": "yes! the word \"husky\" originated from the word referring to arctic people in general, eskimos.", "reference": "yes. huskies got their name from the word referring to eskimos.", "factuality_nli": 2.2996058464050293}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things"], "fact": "it is a spontaneous or gradual process in which old memories are unable to be recalled from memory storage.", "response": "it is a spontaneous or gradual process in which old memories are unable to be recalled from memory storage.", "reference": "its a gradual process where one is unable to call up the older memories", "factuality_nli": 4.014892101287842}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things", "its a gradual process where one is unable to call up the older memories", "yep they just fade away and it can really get to you after a while"], "fact": "problems with remembering, learning and retaining new information are a few of the most common complaints of older adults.", "response": "remembering, learning and retaining new information are a few of the most common complaints of older adults", "reference": "memory problems are one of the most common complaints of older adults", "factuality_nli": 3.544909954071045}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things", "its a gradual process where one is unable to call up the older memories", "yep they just fade away and it can really get to you after a while", "memory problems are one of the most common complaints of older adults", "alzheimer's is one of the worst diseases of all time."], "fact": "many different factors influence the actual process of forgetting.", "response": "many different factors influence the actual process of forgetting", "reference": "alzheimers is terrible but there are many different factors that can affect the process of \"forgetting\"", "factuality_nli": 4.195316314697266}
{"context": ["i think budweiser taste terrible. have you ever had it?"], "fact": "produced in various breweries around the world, budweiser is a filtered beer available in draft and packaged forms.", "response": "budweiser is a filtered beer", "reference": "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "factuality_nli": 3.870133876800537}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company. "], "fact": "in the european union, excluding the united kingdom, republic of ireland, sweden, finland and spain, the american beer is marketed as \"bud\", as the budweiser trademark name is owned solely by the czech beer maker, budweiser budvar.", "response": "yes, and in the european union, excluding the united kingdom, republic of ireland, sweden, finland", "reference": "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "factuality_nli": 0.9145718812942505}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down."], "fact": "budweiser () is an american-style pale lager produced by anheuser-busch, currently part of the transnational corporation anheuser-busch inbev.", "response": "budweiser is an american-style pale lager produced by anheuser-busch", "reference": "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "factuality_nli": 3.9303231239318848}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down.", "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "ah my favorite kind of beer are the stouts. like a nice milk or chocolate stout with a much larger alcohol content. "], "fact": "it is made with up to 30% rice in addition to hops and barley malt.", "response": "i like stouts too! they are made with up to 30% rice in addition to hops and barley malt", "reference": "that sounds yummy!  interestingly, budweiser is made with hops and barley malt, with  up to 30% rice as well", "factuality_nli": -1.6928818225860596}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down.", "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "ah my favorite kind of beer are the stouts. like a nice milk or chocolate stout with a much larger alcohol content.", "that sounds yummy!  interestingly, budweiser is made with hops and barley malt, with  up to 30% rice as well", "oh i didn't know they used rice in their beer. i figured that was all barley, wheat and hops."], "fact": "in 1876, adolphus busch and his friend carl conrad, a liquor importer, developed a \"bohemian-style\" lager in the united states, inspired after a trip to the region.", "response": "interestingly, in 1876, adolphus busch and his friend carl conrad, a liquor importer, developed a bohemian-style lager in the united states", "reference": "yes, and it is a bohemian-style lager developed by adolphus busch and his friend carl conrad", "factuality_nli": 2.708996295928955}
{"context": ["who founded coors brewing company?"], "fact": "in 1873, german immigrants adolph coors and jacob schueler from prussia emigrated to the united states and established a brewery in golden, colorado, after buying a recipe for a pilsner-style beer from a czech immigrant william silhan.", "response": "coors was founded in 1873 by german immigrants adolph coors and jacob schueler.", "reference": "in 1873 adolph coors and jacob schueler founded the brewery", "factuality_nli": 1.6696555614471436}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?"], "fact": "it was first produced in 1978 by the coors brewing company.", "response": "the coors brewing company was first produced in 1978", "reference": "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "factuality_nli": 2.998683214187622}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?", "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "what share of the market for beer did they capture ?"], "fact": "the coors brewing company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "response": "they are a regional division of the world's third-largest brewing company, the molson coors brewing company.", "reference": "i don't know the exact amount but i do know that the company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "factuality_nli": 3.8728859424591064}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?", "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "what share of the market for beer did they capture ?", "i don't know the exact amount but i do know that the company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "wow, that a huge one, thanks for enlightening me about coors brewing company"], "fact": "it is the world's seventh largest brewer by volume.", "response": "it is the world's seventh largest brewer by volume.", "reference": "oh no problem, the molson coors brewing co that was formed in 2005 is now the coors brewing company.", "factuality_nli": 3.9247193336486816}
{"context": ["i love italian cuisine"], "fact": "it has developed through centuries of social and economic changes, with roots stretching to antiquity.", "response": "i love it too! it has developed through centuries of social and economic changes", "reference": "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "factuality_nli": -1.685511589050293}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?"], "fact": "other variations found outside italy may include chicken, veal, or another type of meat cutlet or vegetable filling.", "response": "i like chicken and veal.", "reference": "i really enjoy chicken parmigiana.  what about you?", "factuality_nli": -1.5028536319732666}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?", "i really enjoy chicken parmigiana.  what about you?", "i love chicken parmigiana as well, but i think my ultimate favorite is beef lasagna...extra cheese please!"], "fact": "it consists of a breaded chicken breast topped with tomato sauce and mozzarella, parmesan or provolone cheese.", "response": "oh yes, i love beef parmigiana. what about you?", "reference": "chicken with sauce and mozzarella.... be still my heart!", "factuality_nli": -3.049241542816162}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?", "i really enjoy chicken parmigiana.  what about you?", "i love chicken parmigiana as well, but i think my ultimate favorite is beef lasagna...extra cheese please!", "chicken with sauce and mozzarella.... be still my heart!", "truthfully, anything with cheese is the best"], "fact": "it is the second-most popular cheese in the us (behind mozzarella), with an average annual consumption of per capita.", "response": "cheese is the second most popular cheese in the us.", "reference": "especially cheddar cheese!  it's the second most popular cheese in the us!", "factuality_nli": 3.0164427757263184}
{"context": ["my favorite color is purple, do you know much about that color?"], "fact": "purple is a color intermediate between blue and red.", "response": "i know that it is a color intermediate between blue and red.", "reference": "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "factuality_nli": 0.8976457118988037}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?"], "fact": "according to surveys in europe and the u.s., purple is the color most often associated with royalty, magic, mystery and piety.", "response": "i'm not sure but i do know that purple is associated with royalty, magic, and mystery.", "reference": "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "factuality_nli": -0.7077121734619141}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?", "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "wow that's really neat. do you know what wavelengths of light purple occurs at?"], "fact": "it is similar to violet, but unlike violet, which is a spectral color with its own wavelength on the visible spectrum of light, purple is a composite color made by combining red and blue.", "response": "i do not, but i do know that it is a composite color made by combining red and blue.", "reference": "i'm not sure exactly what wavelengths it occurs at. i do know that purple is similar to violet but unlike that spectral color it is a composite color.", "factuality_nli": -1.2468013763427734}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?", "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "wow that's really neat. do you know what wavelengths of light purple occurs at?", "i'm not sure exactly what wavelengths it occurs at. i do know that purple is similar to violet but unlike that spectral color it is a composite color.", "what exactly is a composite color, can you explain that a bit more?"], "fact": "purple is a color intermediate between blue and red.", "response": "it is a color intermediate between blue and red.", "reference": "composite means that purple is a simple color made by combining red and blue. violet is different because it's spectral.", "factuality_nli": 3.2937192916870117}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd."], "fact": "while the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j.\u00a0r.\u00a0r.\u00a0tolkien, in particular \"the lord of the rings\".", "response": "yeah orcs draw on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j.r.r. tolkien", "reference": "while the concept remains the same it draws on many preexisting mythology", "factuality_nli": 2.2140989303588867}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd.", "while the concept remains the same it draws on many preexisting mythology", "that's really interesting! orcs are some of my favorite fictional characters honestly."], "fact": "while the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j.\u00a0r.\u00a0r.\u00a0tolkien, in particular \"the lord of the rings\".", "response": "the main conception of the creatures stems from the fantasy writings of j. r. r. tolkien", "reference": "orcs were actually created by j r r tolkein", "factuality_nli": 2.4736995697021484}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd.", "while the concept remains the same it draws on many preexisting mythology", "that's really interesting! orcs are some of my favorite fictional characters honestly.", "orcs were actually created by j r r tolkein", "really? cool, i'll have to look him up sometime."], "fact": "an orc (also spelled as ork) is a fictional humanoid creature that is part of a fantasy race akin to goblins.", "response": "orcs are part of a fantasy race akin to goblins", "reference": "orcs are very similar to thinks like goblins and are a humanoid race", "factuality_nli": 3.9365625381469727}

==> example_out_beam/plan-struct-0e.tex <==
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue."], "fact": "the royal blue was the baltimore and ohio railroad (b&o)'s flagship passenger train between new york city and washington, d.c., in the united states, beginning in 1890.", "response": "the royal blue was the baltimore and ohio railroad's flagship passenger train between new york city and washington.", "reference": "i once road on the royal blue train from new york to d.c", "factuality_nli": 3.81148624420166}
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue.", "i once road on the royal blue train from new york to d.c", "oh that sounds really nice. i bet there was a lot of scenery and blue skies."], "fact": "blue skies is a 1946 american musical comedy film directed by stuart heisler and starring bing crosby, fred astaire, and joan caulfield.", "response": "yes, blue skies is a 1946 american musical comedy film directed by stuart heisler", "reference": "yes, speaking of blue skies, have you seen the 1946 movie staring bing crosby?", "factuality_nli": 1.7957786321640015}
{"context": ["blue is my favorite primary color.", "blue is always nice. i like royal blue.", "i once road on the royal blue train from new york to d.c", "oh that sounds really nice. i bet there was a lot of scenery and blue skies.", "yes, speaking of blue skies, have you seen the 1946 movie staring bing crosby?", "no i haven't, but i always like the way he danced."], "fact": "harry lillis \"bing\" crosby jr. (; may 3, 1903\u00a0\u2013 october 14, 1977) was an american singer and actor.", "response": "he was an american singer and actor.", "reference": "yes. i was sad when he died in 1977. he was my favorite actor.", "factuality_nli": 3.4682960510253906}
{"context": ["hi buddy, what you think about cinematography"], "fact": "cinematography (also called \"direction of photography\") is the science or art of motion-picture photography by recording light or other electromagnetic radiation, either electronically by means of an image sensor, or chemically by means of a light-sensitive material such as film stock.", "response": "it is the science or art of motion-picture photography by recording light or other electromagnetic radiation, either electronically by means of an image sensor, or chemically by means of a light-sensitive material such as film stock.", "reference": "cinematography,is a type of motion picture , captured electronically by means of an image", "factuality_nli": 3.9968533515930176}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion."], "fact": "typically, a lens is used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface inside a camera during a questioned exposure, creating multiple images.", "response": "typically, a lens is used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface inside a camera", "reference": "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "factuality_nli": 3.9343953132629395}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", " muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks"], "fact": "photography is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor, or chemically by means of a light-sensitive material such as photographic film.", "response": "photography is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation", "reference": "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "factuality_nli": 4.030572891235352}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks", "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "yes , cinematography finds uses in many fields of science and business as well as for entertainment purposes"], "fact": "a digital camera or digicam is a camera that captures photographs in digital memory.", "response": "a digital camera or digicam is a camera that captures photographs in digital memory", "reference": "some however prefer using   digital camera or digicam ,which is a camera that captures photograph.", "factuality_nli": 3.962085008621216}
{"context": ["hi buddy, what you think about cinematography", "cinematography,is a type of motion picture , captured electronically by means of an image", "yes buddy,  images captured with an electronic image-sensor, produces an electrical charge.the word \"cinematography\" is based on the greek words  meaning movement, motion.", "it works by lens used to repeatedly focus the light reflected from objects into real images on the light-sensitive surface .", "muybridge sequence of a horse galloping in the 1830s, moving images were produced on revolving drums and disks", "cinematography is also a type of photography which is the science, art, application and practice of creating durable images by recording light or other electromagnetic radiation, either electronically by means of an image sensor.", "yes , cinematography finds uses in many fields of science and business as well as for entertainment purposes", "some however prefer using   digital camera or digicam ,which is a camera that captures photograph.", "yes now digital camera is trendy"], "fact": "until the advent of such technology, photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical solutions to develop and stabilize the image.", "response": "until the advent of such technology, photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical solutions to develop and stabilize the image.", "reference": "prior to the advent of digital technology,  photographs were made by exposing light sensitive photographic film and paper, which was processed in liquid chemical .", "factuality_nli": 3.6069302558898926}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?"], "fact": "a genius is a person who displays exceptional intellectual ability, creative productivity, universality in genres or originality, typically to a degree that is associated with the achievement of new advances in a domain of knowledge.", "response": "a genius is a person who displays exceptional intellectual ability, creative productivity, universality in genres or originality, typically to a degree that is associated with the achievement of new advances in a domain of knowledge.", "reference": "universality in genres or originality typically to a degree that is associated with  achievements", "factuality_nli": 4.211020469665527}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?"], "fact": "there is no scientifically precise definition of genius, and the question of whether the notion itself has any real meaning has long been a subject of debate, although psychologists are converging on a definition that emphasizes creativity and eminent achievement.", "response": "there is no scientifically precise definition of genius, and the question of whether the notion itself has any real meaning has long been a subject of debate", "reference": "there is no scientifically precise definition of genius", "factuality_nli": 4.255074501037598}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?", "there is no scientifically precise definition of genius", "are there organizations or anything that you could belong to if you were a genius?"], "fact": "because the achievements of exceptional individuals seemed to indicate the presence of a particularly powerful \"genius\", by the time of augustus, the word began to acquire its secondary meaning of \"inspiration, talent\".", "response": "by the time of augustus, the word began to acquire its secondary meaning of \"inspiration, talent\".", "reference": "the world began to acquire its secondary meaning of inspiration, talent", "factuality_nli": 3.6438181400299072}
{"context": ["a genius is a person who displays exceptional intellectual ability.", "what is an iq of a genius?", "universality in genres or originality typically to a degree that is associated with  achievements", "is that a trait that you can tell someone has early on in their life?", "there is no scientifically precise definition of genius", "are there organizations or anything that you could belong to if you were a genius?", "the world began to acquire its secondary meaning of inspiration, talent", "was albert enstein a genius?"], "fact": "the noun is related to the latin verb \"genui, genitus\", \"to bring into being, create, produce\", as well as to the greek word for birth.", "response": "the noun is related to the latin verb \"genui, genitus\", \"to bring into being, create, produce\"", "reference": "genius word is greed word for birth", "factuality_nli": 3.7850570678710938}
{"context": ["i just got a husky puppy"], "fact": "husky is a general name for a sled-type of dog used in northern regions, differentiated from other sled-dog types by their fast pulling style.", "response": "husky is a general name for a sled-type of dog used in northern regions", "reference": "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "factuality_nli": 3.925452947616577}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?"], "fact": "sled dogs were important for transportation in arctic areas, hauling supplies in areas that were inaccessible by other methods.", "response": "yes, they were important for transportation in the arctic.", "reference": "sled dogs, including huskies, are used for transportation in arctic areas.", "factuality_nli": 2.7909927368164062}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?", "sled dogs, including huskies, are used for transportation in arctic areas.", "that is so cool and probably helpful but mine is just a pet "], "fact": "huskies are also today kept as pets, and groups work to find new pet homes for retired racing and adventure trekking dogs.", "response": "huskies are also kept as pets, and groups work to find new pet homes for retired racing and adventure trekking dogs.", "reference": "that's not uncommon! there are rescue groups that specialize in finding homes for retired sled dogs.", "factuality_nli": 4.213179588317871}
{"context": ["i just got a husky puppy", "it sounds cute! huskies are known amongst sled-dogs for their fast pulling style.", "i guess in the north they are working dogs huh?", "sled dogs, including huskies, are used for transportation in arctic areas.", "that is so cool and probably helpful but mine is just a pet", "that's not uncommon! there are rescue groups that specialize in finding homes for retired sled dogs.", "i bet they retire them at a certain age then they need a home huh"], "fact": "the word \"husky\" originated from the word referring to arctic people in general, eskimos (a.k.a.", "response": "the word \"husky\" originated from the word referring to arctic people in general.", "reference": "yes. huskies got their name from the word referring to eskimos.", "factuality_nli": 3.9551987648010254}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things"], "fact": "it is a spontaneous or gradual process in which old memories are unable to be recalled from memory storage.", "response": "it is a spontaneous or gradual process in which old memories are unable to be recalled from memory storage.", "reference": "its a gradual process where one is unable to call up the older memories", "factuality_nli": 4.014892101287842}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things", "its a gradual process where one is unable to call up the older memories", "yep they just fade away and it can really get to you after a while"], "fact": "problems with remembering, learning and retaining new information are a few of the most common complaints of older adults.", "response": "memory loss is one of the most common complaints of older adults", "reference": "memory problems are one of the most common complaints of older adults", "factuality_nli": 4.008386611938477}
{"context": ["forgetting is the process of losing information already stored in the memory", "yea forgetting and memory loss is one of lifes most painful things", "its a gradual process where one is unable to call up the older memories", "yep they just fade away and it can really get to you after a while", "memory problems are one of the most common complaints of older adults", "alzheimer's is one of the worst diseases of all time."], "fact": "many different factors influence the actual process of forgetting.", "response": "many different factors influence the actual process of forgetting", "reference": "alzheimers is terrible but there are many different factors that can affect the process of \"forgetting\"", "factuality_nli": 4.195316314697266}
{"context": ["i think budweiser taste terrible. have you ever had it?"], "fact": "produced in various breweries around the world, budweiser is a filtered beer available in draft and packaged forms.", "response": "no i haven't. budweiser is produced in various breweries around the world", "reference": "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "factuality_nli": 0.07979893684387207}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company. "], "fact": "in the european union, excluding the united kingdom, republic of ireland, sweden, finland and spain, the american beer is marketed as \"bud\", as the budweiser trademark name is owned solely by the czech beer maker, budweiser budvar.", "response": "yes, in the european union, excluding the united kingdom, republic of ireland, sweden, finland and spain, the american beer is marketed as \"bud\"", "reference": "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "factuality_nli": 3.0281472206115723}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down."], "fact": "budweiser () is an american-style pale lager produced by anheuser-busch, currently part of the transnational corporation anheuser-busch inbev.", "response": "budweiser is an american-style pale lager produced by anheuser-busch", "reference": "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "factuality_nli": 3.9303231239318848}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down.", "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "ah my favorite kind of beer are the stouts. like a nice milk or chocolate stout with a much larger alcohol content. "], "fact": "it is made with up to 30% rice in addition to hops and barley malt.", "response": "i like stouts too! they are made with 30% rice in addition to hops and barley malt", "reference": "that sounds yummy!  interestingly, budweiser is made with hops and barley malt, with  up to 30% rice as well", "factuality_nli": -1.6569770574569702}
{"context": ["i think budweiser taste terrible. have you ever had it?", "yes, and i love it!  it's a filtered beer, and it comes in either draft or packaged forms", "yeah? from my understanding they are called \"bud\" over in europe because they have been in a trademark dispute with another beer company.", "yes, that's true because the trademark name of budweiser is own by the czech beer maker, budweiser budvar", "ah i thought so. i'm not a big fan of theirs because i feel like the beer is really weak and watered down.", "compared to canadian beer, i guess it is!  it is a pale lager though, and is produced by anheuser-busch", "ah my favorite kind of beer are the stouts. like a nice milk or chocolate stout with a much larger alcohol content.", "that sounds yummy!  interestingly, budweiser is made with hops and barley malt, with  up to 30% rice as well", "oh i didn't know they used rice in their beer. i figured that was all barley, wheat and hops."], "fact": "in 1876, adolphus busch and his friend carl conrad, a liquor importer, developed a \"bohemian-style\" lager in the united states, inspired after a trip to the region.", "response": "interestingly, in 1876, adolphus busch and his friend carl conrad, a liquor importer, developed a bohemian-style lager in the united states", "reference": "yes, and it is a bohemian-style lager developed by adolphus busch and his friend carl conrad", "factuality_nli": 2.708996295928955}
{"context": ["who founded coors brewing company?"], "fact": "in 1873, german immigrants adolph coors and jacob schueler from prussia emigrated to the united states and established a brewery in golden, colorado, after buying a recipe for a pilsner-style beer from a czech immigrant william silhan.", "response": "adolph coors and jacob schueler from prussia emigrated to the united states and established a brewery in golden, colorado", "reference": "in 1873 adolph coors and jacob schueler founded the brewery", "factuality_nli": 4.054803371429443}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?"], "fact": "it was first produced in 1978 by the coors brewing company.", "response": "it was first produced in 1978", "reference": "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "factuality_nli": 3.7646842002868652}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?", "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "what share of the market for beer did they capture ?"], "fact": "the coors brewing company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "response": "they are a regional division of the world's third largest brewing company, the molson coors brewing company.", "reference": "i don't know the exact amount but i do know that the company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "factuality_nli": 3.8867685794830322}
{"context": ["who founded coors brewing company?", "in 1873 adolph coors and jacob schueler founded the brewery", "nice, what drinks do they produce?", "i would say one of there most popular items is \"coors light\" which was first produced in 1978, so after 105 years of being founded. but they sell all kinds of beer.", "what share of the market for beer did they capture ?", "i don't know the exact amount but i do know that the company is a regional division of the world's third-largest brewing company, the molson coors brewing company.", "wow, that a huge one, thanks for enlightening me about coors brewing company"], "fact": "it is the world's seventh largest brewer by volume.", "response": "they are the world's seventh largest brewer by volume.", "reference": "oh no problem, the molson coors brewing co that was formed in 2005 is now the coors brewing company.", "factuality_nli": 3.872642993927002}
{"context": ["i love italian cuisine"], "fact": "it has developed through centuries of social and economic changes, with roots stretching to antiquity.", "response": "i love it too. it has developed through centuries of social and economic changes.", "reference": "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "factuality_nli": -1.7194690704345703}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?"], "fact": "other variations found outside italy may include chicken, veal, or another type of meat cutlet or vegetable filling.", "response": "i love anything with meat or vegetables.", "reference": "i really enjoy chicken parmigiana.  what about you?", "factuality_nli": -1.9472707509994507}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?", "i really enjoy chicken parmigiana.  what about you?", "i love chicken parmigiana as well, but i think my ultimate favorite is beef lasagna...extra cheese please!"], "fact": "it consists of a breaded chicken breast topped with tomato sauce and mozzarella, parmesan or provolone cheese.", "response": "i love beef lasagna. it's topped with mozzarella, parmesan or provolone cheese.", "reference": "chicken with sauce and mozzarella.... be still my heart!", "factuality_nli": -0.514546811580658}
{"context": ["i love italian cuisine", "oh yes!  it is the best.  it's really changed over the years but it still has good roots.", "what is your favorite italian dish?", "i really enjoy chicken parmigiana.  what about you?", "i love chicken parmigiana as well, but i think my ultimate favorite is beef lasagna...extra cheese please!", "chicken with sauce and mozzarella.... be still my heart!", "truthfully, anything with cheese is the best"], "fact": "it is the second-most popular cheese in the us (behind mozzarella), with an average annual consumption of per capita.", "response": "cheese is the second most popular cheese in the us!", "reference": "especially cheddar cheese!  it's the second most popular cheese in the us!", "factuality_nli": 2.9982833862304688}
{"context": ["my favorite color is purple, do you know much about that color?"], "fact": "purple is a color intermediate between blue and red.", "response": "i do know that it is a color intermediate between blue and red.", "reference": "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "factuality_nli": 0.5802391171455383}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?"], "fact": "according to surveys in europe and the u.s., purple is the color most often associated with royalty, magic, mystery and piety.", "response": "i don't know much about history but i do know that purple is the color most often associated with royalty, magic, mystery and piety.", "reference": "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "factuality_nli": -1.7551302909851074}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?", "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "wow that's really neat. do you know what wavelengths of light purple occurs at?"], "fact": "it is similar to violet, but unlike violet, which is a spectral color with its own wavelength on the visible spectrum of light, purple is a composite color made by combining red and blue.", "response": "i don't, but i do know that it is similar to violet, but unlike violet, which is a spectral color with its own wavelength on the visible spectrum of light,", "reference": "i'm not sure exactly what wavelengths it occurs at. i do know that purple is similar to violet but unlike that spectral color it is a composite color.", "factuality_nli": -0.931782603263855}
{"context": ["my favorite color is purple, do you know much about that color?", "i don't know much about the color except that it is an intermediate color between blue and red. i do like it though.", "oh that's cool, do you know if purple had any historical uses?", "i would say that it was useful in draping the past royalty of europe and other countries, as well as many magician's ensembles.", "wow that's really neat. do you know what wavelengths of light purple occurs at?", "i'm not sure exactly what wavelengths it occurs at. i do know that purple is similar to violet but unlike that spectral color it is a composite color.", "what exactly is a composite color, can you explain that a bit more?"], "fact": "purple is a color intermediate between blue and red.", "response": "i'm not sure but i do know that purple is a color intermediate between blue and red.", "reference": "composite means that purple is a simple color made by combining red and blue. violet is different because it's spectral.", "factuality_nli": -0.5759638547897339}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd."], "fact": "while the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j.\u00a0r.\u00a0r.\u00a0tolkien, in particular \"the lord of the rings\".", "response": "the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j. r. r. tolkien", "reference": "while the concept remains the same it draws on many preexisting mythology", "factuality_nli": 2.279175281524658}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd.", "while the concept remains the same it draws on many preexisting mythology", "that's really interesting! orcs are some of my favorite fictional characters honestly."], "fact": "while the overall concept of orcs draws on a variety of pre-existing mythology, the main conception of the creatures stems from the fantasy writings of j.\u00a0r.\u00a0r.\u00a0tolkien, in particular \"the lord of the rings\".", "response": "the main conception of the creatures stems from the fantasy writings of j. r. r. tolkien", "reference": "orcs were actually created by j r r tolkein", "factuality_nli": 2.4736995697021484}
{"context": ["orcs are cool fictional humanoid beings", "yeah i've seen them in a lot of things like magic and dnd.", "while the concept remains the same it draws on many preexisting mythology", "that's really interesting! orcs are some of my favorite fictional characters honestly.", "orcs were actually created by j r r tolkein", "really? cool, i'll have to look him up sometime."], "fact": "an orc (also spelled as ork) is a fictional humanoid creature that is part of a fantasy race akin to goblins.", "response": "an orc is a fictional humanoid creature that is part of a fantasy race akin to goblins", "reference": "orcs are very similar to thinks like goblins and are a humanoid race", "factuality_nli": 3.8956902027130127}

==> old-experiments.tex <==

\defcitealias{dinan2018wizard}{Di18}
\defcitealias{shuster2020dialogue}{Sh20}
\defcitealias{rashkin-etal-2021-increasing}{Ra21}
\defcitealias{raffel2020exploring}{Ra20}

\begin{table*}[th!]
\centering
\scalebox{0.65}{
\begin{tabular}{l|ccccccc|ccccccc}
\hline
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{7}{c}{\textbf{Seen Topic}} & \multicolumn{7}{c}{\textbf{Unseen Topic}} \\
& \multicolumn{4}{c}{\textbf{BLEU}} & \textbf{Faithfulness} & \textbf{Coherency} & \textbf{Norm-F1} & \multicolumn{4}{c}{\textbf{BLEU}} & \textbf{Faithfulness} & \textbf{Coherency} & \textbf{Norm-F1} \\ \hline
& \textbf{B1} & \textbf{B2} & \textbf{B3} & \textbf{B4} & & & & \textbf{B1} & \textbf{B2} & \textbf{B3} & \textbf{B4} & & & \\
Reference & $100.0$ & $100.0$ & $100.0$ & $99.99$ & $-0.34$ & $-5.98$ & $23.08$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $-0.3$ & $-5.98$ & $22.54$ \\
Faithful-Oracle & $35.79$ & $20.06$ & $14.36$ & $11.17$ & $3.95$ & $-6.99$ & $0.0$ & $34.71$ & $19.26$ & $13.67$ & $10.46$ & $3.95$ & $-6.88$ & $0.0$ \\
Coherent-Oracle & $4.6$ & $0.57$ & $0.1$ & $0.02$ & $-1.34$ & $-3.59$ & $0.0$ & $4.96$ & $0.57$ & $0.08$ & $0.02$ & $-1.32$ & $-3.52$ & $0.0$ \\ \hline \hline
\makecell[l]{E2E (\citetalias{dinan2018wizard})} & $23.02$ & $7.37$ & $3.48$ & $1.94$ & $-0.37$ & $-5.29$ & $26.92$ & $19.72$ & $3.77$ & $1.15$ & $0.46$ & $-1.56$ & $-5.22$ & $-10.07$ \\
\makecell[l]{Dodeca (\citetalias{shuster2020dialogue})} & $37.76$ & $20.67$ & $14.53$ & $11.18$ & $2.13$ & $-5.84$ & $44.58$ & $38.16$ & $20.68$ & $14.48$ & $11.03$ & $2.16$ & $-5.77$ & $44.02$ \\ \hline
\multicolumn{13}{c}{\textbf{Without Resampling}} \\
T5 (\citetalias{raffel2020exploring}) & $35.56$ & $16.09$ & $10.12$ & $7.25$ & $0.25$ & $-5.51$ & $35.56$ & $35.9$ & $16.32$ & $10.35$ & $7.47$ & $0.37$ & $-5.5$ & $35.97$ \\
ControlCodes (\citetalias{rashkin-etal-2021-increasing}) & $33.17$ & $17.23$ & $11.83$ & $8.94$ & $2.6$ & $-5.88$ & $45.47$ & $32.7$ & $16.65$ & $11.17$ & $8.23$ & $2.6$ & $-5.83$ & $44.06$ \\
PLEDGE-Kw & $36.43$ & $16.85$ & $10.75$ & $7.82$ & $0.6$ & $-5.67$ & $37.75$ & $36.54$ & $16.67$ & $10.67$ & $7.7$ & $0.57$ & $-5.59$ & $37.09$ \\
PLEDGE-St & $33.65$ & $16.87$ & $11.38$ & $8.48$ & $2.19$ & $-5.78$ & $46.52$ & $33.92$ & $16.77$ & $11.15$ & $8.22$ & $2.2$ & $-5.71$ & $45.78$ \\
PLEDGE-Full & $34.69$ & $16.35$ & $10.46$ & $7.55$ & $1.38$ & $-5.61$ & $45.48$ & $34.68$ & $16.2$ & $10.3$ & $7.39$ & $1.42$ & $-5.61$ & $43.81$ \\ \hline
\multicolumn{13}{c}{\textbf{With Resampling}} \\
T5 (\citetalias{raffel2020exploring}) & $34.81$ & $15.79$ & $9.81$ & $6.94$ & $1.55$ & $-4.79$ & $59.23$ & $35.18$ & $15.97$ & $9.98$ & $6.99$ & $1.59$ & $-4.77$ & $58.82$ \\
ControlCodes (\citetalias{rashkin-etal-2021-increasing}) & $33.11$ & $17.48$ & $11.85$ & $8.87$ & $3.27$ & $-5.25$ & $64.67$ & $32.9$ & $16.75$ & $11.12$ & $8.09$ & $3.24$ & $-5.17$ & $64.04$ \\
PLEDGE-Kw & $36.12$ & $16.8$ & $10.6$ & $7.61$ & $1.73$ & $-5.03$ & $57.83$ & $35.91$ & $16.55$ & $10.45$ & $7.36$ & $1.74$ & $-4.92$ & $58.22$ \\
PLEDGE-St & $33.72$ & $16.89$ & $11.24$ & $8.24$ & $2.99$ & $-5.1$ & $66.26$ & $33.88$ & $16.73$ & $10.88$ & $7.86$ & $2.99$ & $-5.01$ & $66.23$ \\
PLEDGE-Full & $34.92$ & $16.54$ & $10.56$ & $7.55$ & $2.15$ & $-5.0$ & $61.99$ & $34.72$ & $16.16$ & $10.21$ & $7.24$ & $2.21$ & $-4.97$ & $61.41$ \\ \hline
\end{tabular}}
\caption{\label{tab:wow_test_results} Results on the seen/unseen portions of the Wizard of Wikipedia test set. Resampling is performed by sampling $10$ responses and re-ranking them based on the average of faithfulness and coherency rankings. All PLEDGE models use $3$ rounds of edits using the editor E. Higher is better for all metrics. Numbers in \textbf{{\color{blue}blue}} and \textbf{{\color{red}red}} represent the best and worst performance among the trained models respectively.}
\end{table*}

\begin{table*}[th!]
\centering
\scalebox{0.65}{
\begin{tabular}{l|ccccccc|ccccccc}
\hline
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{7}{c}{\textbf{Topical Chat}} & \multicolumn{7}{c}{\textbf{CMU-DoG}} \\
& \multicolumn{4}{c}{\textbf{BLEU}} & \textbf{Faithfulness} & \textbf{Coherency} & \textbf{Norm-F1} & \multicolumn{4}{c}{\textbf{BLEU}} & \textbf{Faithfulness} & \textbf{Coherency} & \textbf{Norm-F1} \\ \hline
& \textbf{B1} & \textbf{B2} & \textbf{B3} & \textbf{B4} & & & & \textbf{B1} & \textbf{B2} & \textbf{B3} & \textbf{B4} & & & \\
Reference & & & & & & & & & & & & & & \\
Faithful-Oracle & & & & & & & & & & & & & & \\
Coherent-Oracle & & & & & & & & & & & & & & \\ \hline \hline
\multicolumn{13}{c}{\textbf{Without Resampling}} \\
T5 (\citetalias{raffel2020exploring}) & & & & & & & & & & & & & & \\
ControlCodes (\citetalias{rashkin-etal-2021-increasing}) & & & & & & & & & & & & & & \\
PLEDGE-Kw & & & & & & & & & & & & & & \\
PLEDGE-St & & & & & & & & & & & & & & \\
PLEDGE-Full & & & & & & & & & & & & & & \\ \hline
\multicolumn{13}{c}{\textbf{With Resampling}} \\
T5 (\citetalias{raffel2020exploring}) & & & & & & & & & & & & & & \\
ControlCodes (\citetalias{rashkin-etal-2021-increasing}) & & & & & & & & & & & & & & \\
PLEDGE-Kw & & & & & & & & & & & & & & \\
PLEDGE-St & & & & & & & & & & & & & & \\
PLEDGE-Full & & & & & & & & & & & & & & \\ \hline
\end{tabular}}
\caption{\label{tab:tc_cmu_test_results} Results on the seen portions of the Topical Chat and CMU-DoG test sets. Resampling is performed by sampling $10$ responses and re-ranking them based on the average of faithfulness and coherency rankings. All PLEDGE models use $3$ rounds of edits using the editor E. Higher is better for all metrics.}
\end{table*}

Overview - key objective to use the PLEDGE framework to handle coherency-factuality trade-off in knowledge-grounded dialogues. Since we have a lot of analysis in mind, organize in the form of research questions as in Section 5 here: https://arxiv.org/pdf/2205.00344.pdf

So may be three questions can be: 1) How useful is the proposed methodology to generate responses with improved Q - here we look at automatic evaluations, scatter plot, and analysis that emphasizes on the performance, 2) How do these findings compare to human annotators - where we show human eval, 3) Error Analysis: What errors does the model make, key challenges, and sources of improvement? - where the analysis is done to understand the model behavior and guide future work.

We first describe the experimental setup and then discuss results to answer the above questions.

Data: Describe wow + give data split.

Plan variables: describe structural and lexical variables + how they are all computed - can move a lot of this to appendix.

We turn to prior work and explore a number of plan variables. we define two broad categories that the prior work has explored - structural + lexical ..We experiment with both these kinds of variables in this paper and further create a full model that uses them in conjunction.

Plan variables: show the data preprocessing for an actual example from the wow dataset in Appendix (already in internship slides). - after introducing the plan variables.

then, we add about what plan variables are etc.

Quality Estimators: faithfulness - begin nli, coherency- briefly discuss the challenges to capture coherence - give two examples comparing reference vs fact scores for different metrics that you considered - push to appendix. can use a bar-graph here. Then say that we use --> DGPT.

A lot of the detail about what the quality estimators are - what our goal is - will be discussed here instead e.g. stuff in Section 2 here: https://arxiv.org/pdf/2107.06963.pdf

Baselines and Ablations: Seq2Seq, Control Codes, PLEDGE, PLEDGE-No Edits (this captures prior planning approaches), PLEDGE-S (only struct vars), PLEDGE-L (only lexical vars), - there are no baselines that incorporate both the metrics so this is not fair yet.

Other baselines

- may be one method that uses some dummy heuristic (like dropping entities keywords) just to capture some heuristic approaches in the prior work - may not add value
- Resampling approach
- PLEDGE + Resampling approach (may be this should be a part of PLEDGE - oh yes) and then resampling is like an ablation.
- Factuality-oracle: just use the fact directly.
- Coherency-oracle: ask DGPT to output a sentence

So a lot of the prior work seems to be covered in these right - reranking/resampling is popular which can incorporate more than one metric, then planning is popular (without editing) - then just optimizing for one metric. - any other approach that we should build which incorporates both the metrics? - probably not required but lets look at the related work.

All these combined seem to be enough I guess.

PLEDGE training details

Based on the neural seq2seq architecture T5, that has been widely applied across dialogue and other NLP applications [CITES].

Hyperparameters - in brief for both G and E models. - or move to Appendix.

Data, plan variables, oracle metrics, compared models (baselines) + hyperparameters in brief (rest move to appendix), evaluation measures (intrinsic + extrinsic)

automated evaluation results (intrinsic/extrinsic): intrinsic plan-specific metrics (okay on val data), scatter plot, human evaluation results, error analysis/qualitative examples: How the plans are being changed, number of edits performed (val data), vary the type of data used for training the editing models, varying the decoding strategy for the full model, varying the metric on which the editing models are trained, discuss interesting validation examples (creative solutions like yes, and type work), any editing issues that you faced - and discuss future work to fix them.

Make result tables, Figure templates - with dummy bar graphs, etc.


==> orig_plan_editor_section.tex <==
During inference, the base model $G$ described above is capable of both planning and response generation. However, this is insufficient by itself in cases where the training data does not fully satisfy the quality constraints set by $Q$. This can especially be true for knowledge-grounded dialogues where not all ground-truth responses are fully attributable to the input evidence~\cite{dziri2022origin}. Further, it is challenging to achieve the desired quality in a post-processing step, once the response is already generated. Hence, to tackle this, we propose an editor that performs this editing at the level of content plans, which then guides $G$ to produce the final output contextually.

Formally, the editor $E_{Q}$ takes in the candidate plan sequence $\hat{c}$, along with conversation history $x$ and evidence $e$, and generates the modified plan $\hat{c}'$ to better satisfy the quality estimator $Q$. To design our editor $E_{Q}$, we adapt the MASKER text editing approach from style transfer literature~\cite{malmi2020unsupervised}. Text editing methods convert the task of seq2seq generation into sequence editing, which helps in efficiency especially in the cases with high input-output overlap. Further, MASKER provides an unsupervised way to perform the editing by training a unified non-autoregressive model without needing to define explicit edit operations and generating synthetic parallel data. This is especially useful for our scenario since the dialogue quality metrics that capture constraints such as factuality and coherency work at the response-level, making it challenging to obtain parallel data for plan-to-plan generation.  

Assume access to source domain data ($\Theta_{\textrm{source}}$) and target domain data ($\Theta_{\textrm{target}}$). $\Theta_{\textrm{source}}$ and $\Theta_{\textrm{target}}$ essentially corresponding to the poor and good quality plans respectively, as per the estimator $Q$. In our experiments, this data comes from three sources: 1) Using low and high quality samples from the training data, as measured by $Q$, 2) Using a similar split on other related knowledge-grounded dialogue datasets, and 3) By performing perturbations for data augmentation and then assigning them to $\Theta_{\textrm{source}}$ or $\Theta_{\textrm{target}}$ based on $Q$.

\noindent\textbf{Training}: Following MASKER, we train a non-autoregressive language model~\cite{liu2019roberta} using the Padded Masked Language Modeling (MLM) strategy~\cite{mallinson2020felix}. Padded MLM modifies the original MLM objective to also take into account the length of infilled tokens. Instead of masking a single token, this approach masks out sequence of whole words up to $n_p$ tokens. The remaining tokens are filled with [PAD] to ensure that the input always consists of $n_p$ [MASK] tokens. Then, the model is trained on the pseudo-likelihood of the original tokens $C_{i:j}$:
\begin{multline}
    L(C_{i:j} | C_{\textbackslash i:j};\Theta) = \prod_{t=i}^{j}P_{MLM}(c_t | C_{\textrm{\textbackslash} i:j};\Theta)\\ \times \prod_{t=j+1}^{i+n_p-1}P_{MLM}([PAD]_t | C_{\textrm{\textbackslash} i:j};\Theta) 
\end{multline}
$i:j$ denotes the original tokens that are masked in the sequence $C$. $P_{MLM}(c_t | C_{\textrm{\textbackslash} i:j};\Theta)$ is the probability of the random variable corresponding to the t-th token in $C_{\textrm{\textbackslash} i:j}$ taking the value $c_t$ or [PAD]. Finally, $\Theta$ corresponds to either $\Theta_{\textrm{source}}$ or $\Theta_{\textrm{target}}$, depending on the data the model is trained on. In practice, a single unified model is trained by using a special indicator token [SOURCE] or [TARGET] in the input.  

\noindent\textbf{Inference}: For inference, the editor model needs to find a text span where the source and the target models disagree the most and then replace this with the maximum likelihood replacement suggested by the target model $\hat{C_{i:j}}^{\textrm{target}}$. Since the content plans are relatively shorter than entire utterances and bounded, we try out all the possible masking positions $i:j$ in order to maximize the score $S(i,j)$:

%, while still keeping the total masked length to $n_p$ using [PAD] tokens. The final position is decided by the score $S(i,j)$: 

\begin{equation}
    S(i,j) = TS(i,j) + SS(i,j),
\end{equation}
\begin{multline}
TS(i,j) = L(\hat{C_{i:j}}^{\textrm{target}} | C_{\textrm{\textbackslash} i:j};\Theta_{\textrm{target}}) \\ - L(C_{i:j} | C_{\textrm{\textbackslash} i:j};\Theta_{\textrm{target}})
\end{multline}
\begin{multline}
SS(i,j) = -\textrm{max}[0, L(\hat{C_{i:j}}^{\textrm{target}} | C_{\textrm{\textbackslash} i:j};\Theta_{\textrm{source}}) \\ - L(C_{i:j} | C_{\textrm{\textbackslash} i:j};\Theta_{\textrm{source}})]
\end{multline}

$TS(i,j)$ is the score computed with respect to the target model. Intuitively, a position is preferable if a) a good replacement is available, and b) the existing tokens are less likely under the target model.

The term $SS(i,j)$ evaluates $\hat{C_{i:j}}^{\textrm{target}}$ and $C_{i:j}$ under the source model. \gt{can we give abetter justification for SS} It is used as a check for the cases when the target model is overly confident by mistake, such as replacing rare entities with more common ones which may not necessarily help to improve the quality of a content plan (w.r.t $Q$).

% Our implementation differs from the original MASKER model in three primary aspects: 1) We use partial editing, where  only on the planning sequence, 2) use roberta -> tokenizer is simpler to modify for padded MLM, 3) Instead of pretraining the model, we perform joint learning with multiple datasets and introduce perturbations for data augmentation.


% Post-hoc resampling: Also discuss the resampling approach as required. Note that this is complementary to our approach which performs edits at the plan-level. This takes care of the decoding time sampling methods - complementary to our approach.

% Describe params separately - like this: LEWIS: https://aclanthology.org/2021.findings-acl.344.pdf and MASKER: https://arxiv.org/pdf/2010.01054.pdf

% three types of phi -> E target, E source, G

% A figure that clearly shows the inputs and the output formats. Use notation similar to the figure here: https://arxiv.org/pdf/2107.06963.pdf

% Input format: 

% Editing Model E

% Format for the editing model + plan (can just use input tokens here) ..use a figure that at a higher-level shows what happens for training and editing. Train: mask out and predict, Test: Mask out, measure disagreement, suggest alternative - a higher-level figure is fine I guess with MASKER described in text from here: https://arxiv.org/pdf/2010.01054.pdf

% Ending comments: 

% Explain that this approach is inspired from some of the heuristics which perform edits at the level of plans - but want to automate it.

% Explain that although described in the context of knowledge-grounded dialogue, the approach is generic and can be applied to other text generation scenarios by defining appropriate planning variables.

==> table_beam_search.tex <==

\begin{table*}[th!]
\centering
\scalebox{0.65}{
\begin{tabular}{l|ccccccc|ccccccc}
\hline
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{7}{c}{\textbf{Seen Topic}} & \multicolumn{7}{c}{\textbf{Unseen Topic}} \\
& \multicolumn{4}{c}{\textbf{BLEU}} & \textbf{Faithfulness} & \textbf{Coherency} & \textbf{Norm-F1} & \multicolumn{4}{c}{\textbf{BLEU}} & \textbf{Faithfulness} & \textbf{Coherency} & \textbf{Norm-F1} \\ \hline
& \textbf{B1} & \textbf{B2} & \textbf{B3} & \textbf{B4} & & & & \textbf{B1} & \textbf{B2} & \textbf{B3} & \textbf{B4} & & & \\
Reference & $100.0$ & $100.0$ & $100.0$ & $99.99$ & $-0.34$ & $-5.98$ & $23.08$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $-0.3$ & $-5.98$ & $22.54$ \\
Faithful-Oracle & $35.79$ & $20.06$ & $14.36$ & $11.17$ & $3.95$ & $-6.99$ & $0.0$ & $34.71$ & $19.26$ & $13.67$ & $10.46$ & $3.95$ & $-6.88$ & $0.0$ \\
Coherent-Oracle & $4.6$ & $0.57$ & $0.1$ & $0.02$ & $-1.34$ & $-3.59$ & $0.0$ & $4.96$ & $0.57$ & $0.08$ & $0.02$ & $-1.32$ & $-3.52$ & $0.0$ \\ \hline \hline
\makecell[l]{E2E (\citetalias{dinan2018wizard})} & $23.02$ & $7.37$ & $3.48$ & $1.94$ & $-0.37$ & $-5.29$ & $26.92$ & $19.72$ & $3.77$ & $1.15$ & $0.46$ & $-1.56$ & $-5.22$ & $-10.07$ \\
\makecell[l]{Dodeca (\citetalias{shuster2020dialogue})} & $37.76$ & $20.67$ & $14.53$ & $11.18$ & $2.13$ & $-5.84$ & $44.58$ & $38.16$ & $20.68$ & $14.48$ & $11.03$ & $2.16$ & $-5.77$ & $44.02$ \\
T5 (\citetalias{raffel2020exploring}) & 35.52 & 19.44 & 13.705 & 10.591 & 2.04 & -5.68 & 48.1 \\
ControlCodes (\citetalias{rashkin-etal-2021-increasing}) &33.3& 18.71& 13.46 & 10.54 & 3.22 & -5.98 & 44.2 \\ \hline
\multicslumn{13}{c}{\textbf{Plans Without Editing}} \\
PLEDGE-Kw+0e  & 35.10 & 19.03 & 13.31 & 10.28 & 1.81  & -5.74 & 45.5 \\
PLEDGE-St+0e& 36.66 & 19.60 & 13.72 & 10.51 & 1.53 & -5.60 & 46.6 \\
PLEDGE-Full+0e & 33.52 & 17.72 & 12.25 & 9.29 & 1.41 & -5.61 & 45.6 \\ \hline
\multicolumn{13}{c}{\textbf{Plans With Editing}} \\
PLEDGE-Kw+1e &0.33576 &0.18477 &0.13035& 0.10105 & 2.14 &  -5.70 & 48.1 & & & & & & & \\ 
PLEDGE-St+1e &0.33437 &0.18643 &0.13317& 0.10374  & 2.69 & -5.82 & 47.4 & & & & & \\
PLEDGE-Full+1e & 0.30405& 0.16253& 0.1134 &0.08653 & 1.77 & -5.61 & 48.0& & & & & & & \\ \hline
PLEDGE-Kw+3e & & & & &   & & & & & & & & & \\
PLEDGE-St+3e & & & & & 2.89 & & & & & & & & & \\
PLEDGE-Full+3e & 0.30745 & 0.16486& 0.11586 & 0.08884 & 2.04 & & & & & & & & & \\ \hline
PLEDGE-Kw+9e & 0.34034 0.18675 0.13163 0.1019 & 2.15 & -5.70 & 47.9 & & & & & & & \\
PLEDGE-St+9e  & 0.33147 0.18554 0.13261 0.10321 & 2.90 & -5.79 & 49.0  & & & & & & & & & \\
PLEDGE-Full+9e & 0.30915 0.16603 0.1167 0.08945 & 2.09 & -5.69 & 48.1& & & & & & & \\ \hline
\end{tabular}}
\caption{\label{tab:tc_cmu_test_results} Results on the seen portions of the Topical Chat and CMU-DoG test sets. Resampling is performed by sampling $10$ responses and re-ranking them based on the average of faithfulness and coherency rankings. All PLEDGE models use $3$ rounds of edits using the editor E. Higher is better for all metrics.}
\end{table*}
